Unsupervised Domain Adaptation for Hate Speech Detection Using a Data Augmentation Approach

Online harassment in the form of hate speech has been on the rise in recent years. Addressing the issue requires a combination of content moderation by people, aided by automatic detection methods. As content moderation is itself harmful to the people doing it, we desire to reduce the burden by improving the automatic detection of hate speech. Hate speech presents a challenge as it is directed at different target groups using a completely different vocabulary. Further the authors of the hate speech are incentivized to disguise their behavior to avoid being removed from a platform. This makes it difficult to develop a comprehensive data set for training and evaluating hate speech detection models because the examples that represent one hate speech domain do not typically represent others, even within the same language or culture. We propose an unsupervised domain adaptation approach to augment labeled data for hate speech detection. We evaluate the approach with three different models (character CNNs, BiLSTMs and BERT) on three different collections. We show our approach improves Area under the Precision/Recall curve by as much as 42% and recall by as much as 278%, with no loss (and in some cases a significant gain) in precision.

==> datasets.tex <==
\section{Hate Speech Datasets}\label{data}
\sheikh{Need to rewrite. Everything is copied. We will be charged with Plagiarism. }
In the following paragraphs we discuss about several hate speech datasets:

\subsection{Hate Speech Dataset from a White Supremacy Forum} The annotated sentences of this dataset have been extracted from Stormfront, a white supremacist forum. Stormfront is the largest online community of white nationalists, characterised by pseudo-rational discussions of race. 

A total number of 10,568 sentences have been extracted from Stormfront and classified as conveying hate speech or not, and into two other auxiliary classes. In addition, the following information is also given for each sentence: a post identifier and the sentence’s position in the post, a user identifier, a sub-forum identifier. This information makes it possible re-build the conversations
these sentences belong to.

The extracted forum content was published between 2002 and 2017. The process of preparing the candidate content to be annotated was the following: 

\begin{itemize}
    \item A subset of 22 sub-forums covering diverse topics and nationalities was random-sampled
    to gather individual posts uniformly distributed among sub-forums and users. 
    
    \item The sampled posts were filtered using an automatic language detector to discard non-English texts.
    
    \item The resulting posts were segmented into sentences with ixapipes. 
    
    \item The sentences were grouped forming batches of 500 complete posts (1,000 sentences per batch).

\end{itemize}

\subsubsection{Annotation Process} In this study, all the annotators together created and discussed the guidelines to ensure all participants had the same understanding of hate speech. The final guidelines consider 4 types of sentences.

\paragraph{HATE} Sentences in this category contain hate speech. Hate speech is a: 

\begin{itemize}
    \item deliberate attack
    \item directed towards a specific group of people
    \item motivated by aspects of the group’s identity.
\end{itemize}

Some examples from the HATE class are: 

\begin{itemize}
    \item Poor white kids being forced to treat apes and parasites as their equals.
    \item Islam is a false religion however unlike some other false religions it is crude and appeals to crude people such as arabs.
\end{itemize}

\paragraph{NOHATE} This label is used to categorise sentences that do not convey hate speech per the established definition.

\begin{itemize}
    \item Where can I find NS speeches and music, also historical, in mp3 format for free download on the net.
    \item I know of Chris Rock and subsequently have hated him for a long time. 
\end{itemize}

The second sentence is not a hate speech becuase it is a personal attack, not against a group based on their properties. Finally, it must be emphasized that the presence of pejorative language in a sentence cannot systematically be considered sufficient evidence to confirm the existence of hate speech. The use of “fag” in the following sentence: 

``Two black fag’s holding hands.''

cannot be said to be a deliberate attack, taken without any more context, despite it likely being offensive. Therefore, it cannot be considered HATE.

\paragraph{RELATION} Consider an example:

\begin{itemize}
    \item Probably the most disgusting thing I’ve seen in the last year.
    \item She looks like she has some African blood in her, or maybe it’s just the makeup.
    \item This is just so wrong.
\end{itemize}

Each sentence in isolation does not convey hate speech: in 1 and 3, a negative attitude is perceived, but it is unknown whether it is targeted towards a group of people; in 2, there is no
hint of an attack, not even of a negative attitude. However, the three sentences together suggest that having “African blood” makes a situation (whatever “this” refers to) disgusting, which constitutes hate speech according to the definition proposed. The label RELATION is given  separately to all the sentences that need each other to be understood as hate speech.

\paragraph{SKIP} 
Sentences that are not written in English or that do not contain information as to be classified into HATE or NOHATE are given this label.


All the annotation work was carried out using a web-based tool developed by the authors for this purpose. The tool displays all the sentences belonging to the same post at the same time, giving the annotator a better understanding of the post’s author’s intention. If the complete post is deemed insufficient by the annotator to categorize a sentence, the tool can show previous posts to which the problematic post is answering, on demand, up to the first post in the thread and its title. 

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{gibert_stat.png}
    \caption{Dataset Statistic \cite{de-gibert-etal-2018-hate}}
    \label{fig:my_label}
\end{figure}


\subsection{Hateful Symbols or Hateful People?Predictive Features for Hate Speech Detection on Twitter}

Our data set consists of tweets collected over the course of 2 months. In total, we retrieved 136,052 tweets and annotated 16,914 tweets, 3,383 of that for  sexist  content  sent  by  613  users,  1,972  for racist content sent by 9 users, and 11,559 for neither sexist or racist and is sent by 614 users. Since  hate  speech  is  a  real,  but  limited  phenomenon, we do not balance the data, to provide as realistic a data set as possible.

We bootstrapped our corpus collection, by performing an initial manual search of common slurs and terms used pertaining to religious, sexual, gender, and ethnic minorities. In the results,  we  identified  frequently  occurring  terms in tweets that contain hate speech and references to specific entities, such as the term ``\#MKR''. All  terms  queried  for:   ``MKR'',  ``asian  drive'',  ``femi-nazi'',  ``immigrant'',  ``nigger'',  ``sjw'',  ``WomenAgainstFem-inism'',  ``blameonenotall'',  ``islam  terrorism'',  ``notallmen'', ``victimcard'',   ``victim  card'',   ``arab  terror'',   ``gamergate'', ``jsil'', ``racecard'', ``race card''.

Based on this sample, we used the public Twitter search API to collect the entire corpus, filtering for  tweets  not  written  in  English.   This  particular  corpus  construction  ensures  that  we  obtain non-offensive tweets that contain both clearly offensive words and potentially offensive words, but remain non-offensive in their use and treatment of the words.  For example, even though ``muslims'' is one of the most frequent words in racist tweets,it also occurs in perfectly innocuous tweets, such as ``you are right there are issues but banning Muslims from entering does not solve anything.''

We manually annotated our data set, after which we had the help of an outside annotator (a 25 year old  woman  studying  gender  studies  and  a  non-activist feminist) to review our annotations, in order to mitigate annotator bias introduced by any parties.

We  propose  the  following  list  to  identify  hate speech. The criteria are partially derived by negating  the  privileges  observed  in  McIntosh  (2003), where they occur as ways to highlight importance, ensure  an  audience,  and  ensure  safety  for  white people, and partially derived from applying common sense. 

A tweet is offensive if it has the following properties:

\begin{itemize}
    \item uses a sexist or racial slur.
    \item attacks a minority.
    \item seeks to silence a minority.
    \item criticizes a minority (without a well founded argument)
    \item promotes,  but  does  not  directly  use,  hate speech or violent crime.
    \item criticizes a minority and uses a straw man argument.
    \item blatantly misrepresents truth or seeks to distort  views  on  a  minority  with unfounded claims.
    \item shows support of problematic hash tags. E.g. ``\#BanIslam'',  ``\#whoriental'',  ``\#whitegeno-cide''
    \item negatively stereotypes a minority.10.  defends xenophobia or sexism.
    \item contains a screen name that is offensive,  as per the previous criteria, the tweet is ambiguous (at best), and the tweet is on a topic that satisfies any of the above criteria.
\end{itemize}


The inter-annotator agreement is $\kappa$ = 0.84.85\% of all disagreements occur  in  annotations  of  sexism,  with 98\%  of  all reviewer  changes  being  set  to  neither  sexist  nor racist, the remaining set to racist. In most of these cases we find that the disagreement is reliant on context or the lack thereof.

\subsection{Automated Hate Speech Detection and the Problem of Offensive Language}
We begin with a hate speech lexicon containing words and phrases identified by internet users as hate speech, compiled by Hatebase.org. Using the Twitter API we searched for tweets containing terms from the lexicon, resulting in a sample of tweets from 33,458 Twitter users. We extracted the timeline for each user, resulting in a set of 85.4 million tweets. From this corpus we then took a random sample of 25k tweets containing terms from the lexicon and had them manually coded by CrowdFlower (CF) workers. Workers were asked to label each tweet as one of three categories: hate speech, offensive but not hate speech, or neither offensive nor hate speech. They were provided with our definition along with a paragraph explaining it in further detail. Users were asked to think not just about the words appearing in a given tweet but about the context in  which they were used. They were instructed that the presence of a particular word, however offensive, did not necessarily indicate a tweet is hate speech. Each tweet was coded by three or more people. The inter-coder agreement score provided by CF is 92\%. We use the majority decision for each tweet to assign a label. Some tweets were not assigned labels as there was no majority class. This results in a sample of 24,802 labeled tweets. Only 5\% of tweets were coded as hate speech by the majority of coders and only 1.3\% were coded unanimously,demonstrating the imprecision of the Hatebase lexicon. This is much lower than a comparable study using Twitter, where 11.6\% of tweets were flagged as hate speech, likely because we use a stricter criteria for hate speech. The majority of the tweets were considered to be offensive language (76\% at 2/3, 53\% at 3/3) and the remainder were considered to be non-offensive (16.6\% at 2/3, 11.8\% at 3/3). We then constructed features from these tweets and used them to train a classifier. 

We lower cased each tweet and stemmed it using the Porter stemmer,3then create bigram, unigram, and trigram features, each weighted by its TF-IDF. To capture information about the syntactic structure we use NLTK to construct Penn Part-of-Speech (POS) tag unigrams, bigrams, and trigrams. To capture the quality of each tweet we use modified Flesch-Kincaid Grade Level and Flesch Reading Ease scores, where the number of sentences is fixed at one. We also use a sentiment lexicon designed for social media to assign sentiment scores to each tweet. We also include binary and count indicators for hashtags, mentions, retweets, and URLs, as well as features for the number of characters, words, and syllables in each tweet.

\subsection{Multilingual Detection of Hate Speech Against Immigrants and Women in Twitter}

\subsubsection{Data} The data have been collected using different gathering strategies. For what concerns the time frame,tweets  have  been  mainly  collected  in  the  timespan from July to September 2018,  with the exception  of  data  with  target  women.   Indeed,  the most  part  of  the  training  set  of  tweets  against women has been derived from an earlier collection carried  out  in  the  context  of  two  previous  challenges on misogyny identification. Different  approaches  were  employed to  collect  tweets:   (1)  monitoring  potential  victims  of  hate  accounts,  (2)  downloading  the  history  of  identified  haters  and  (3)  filtering  Twitter streams with keywords, i.e.  words, hashtags and stems.   Regarding  the  keyword-driven  approach,we employed both neutral keywords, derogatory words against the targets, and highly polarized hashtags, in order to collect a cor-pus for reflecting also on the subtle but important differences between HS, offensiveness and stance.  The keywords  that  occur  more  frequently  in  the  collected  tweets  are:migrant,refugee,\#buildthatwall, bitch, hoe, women for English, and inmigra-, arabe, sudaca, puta, callate, perra for Spanish.

The  entire  HatEval  dataset  is  composed  of 19,600 tweets,  13,000 for English and 6,600 for Spanish. They are distributed across the targets as follows: 9,091 about immigrants and 10,509 about women. It includes the following categories:

\begin{itemize}
    \item HS- a binary value indicating if HS is occur-ring against one of the given targets (women or immigrants): 1 if occurs, 0 if not.
    
    \item Target Range- if HS occurs (i.e.  the value for the feature HS is 1), a binary value indicating if the target is a generic group of people (0) or a specific individual (1).
    
    \item Aggressiveness- if HS occurs (i.e. the value for  the  feature  HS  is  1),  a  binary  value  indicating  if  the  tweeter  is  aggressive  (1) or not (0).
    
\end{itemize}

According to the schema described above,  the format of an annotated tweet in the training and development set has the following pattern:ID, Tweet-text, HS, TR, AG where  ID  is  a  progressive  number  denoting  the tweet  within  the  dataset,  Tweet-text  is  the  given text of the tweet, while the other parts of the pat-tern, given in the training data and to be predicted in the test set, are: Hate Speech [HS] (1 or 0), Target Range [TR] (0 for group or 1 for individual),and Aggressiveness [AG] (0 or 1).  Data included in the test instead only include ID and Tweet-text,the annotation of HS, TR and AG to be provided by participants according to the subtask.


